Multi-Agent Search-Type Problems on Polygons

We present several advancements in search-type problems for fleets of mobile agents operating in two dimensions under the wireless model. Potential hidden target locations are equidistant from a central point, forming either a disk (infinite possible locations) or regular polygons (finite possible locations). Building on the foundational disk evacuation problem, the disk priority evacuation problem with $k$ Servants, and the disk $w$-weighted search problem, we make improvements on several fronts. First we establish new upper and lower bounds for the $n$-gon priority evacuation problem with $1$ Servant for $n \leq 13$, and for $n_k$-gons with $k=2, 3, 4$ Servants, where $n_2 \leq 11$, $n_3 \leq 9$, and $n_4 \leq 10$, offering tight or nearly tight bounds. The only previous results known were a tight upper bound for $k=1$ and $n=6$ and lower bounds for $k=1$ and $n \leq 9$. Second, our work improves the best lower bound known for the disk priority evacuation problem with $k=1$ Servant from $4.46798$ to $4.64666$ and for $k=2$ Servants from $3.6307$ to $3.65332$. Third, we improve the best lower bounds known for the disk $w$-weighted group search problem, significantly reducing the gap between the best upper and lower bounds for $w$ values where the gap was largest. These improvements are based on nearly tight upper and lower bounds for the $11$-gon and $12$-gon $w$-weighted evacuation problems, while previous analyses were limited only to lower bounds and only to $7$-gons.

==> UpperBoundsFigs/k3servants/3gonk3fig.tex <==
\begin{figure}[h!]
\caption{A search trajectory for \pe{3}{3}. 
Trajectory details can be found in Table~\ref{3gonk3tab}.}
\label{3gonk3fig}
\end{figure}

==> UpperBoundsFigs/k4servants/10gonk4fig.tex <==
\begin{figure}[h!]
\caption{A search trajectory for \pe{10}{4}. 
Trajectory details can be found in Table~\ref{10gonk4tab}.}
\label{10gonk4fig}
\end{figure}

==> UpperBoundsFigs/k4servants/3gonk4fig.tex <==
\begin{figure}[h!]
\caption{A search trajectory for \pe{3}{4}. 
Trajectory details can be found in Table~\ref{3gonk4tab}.}
\label{3gonk4fig}
\end{figure}

==> UpperBoundsFigs/k4servants/4gonk4fig.tex <==
\begin{figure}[h!]
\caption{A search trajectory for \pe{4}{4}. 
Trajectory details can be found in Table~\ref{4gonk4tab}.}
\label{4gonk4fig}
\end{figure}

==> UpperBoundsTabs/k2servants/9gonk2tab-old.tex <==
\begin{table}[h!]
\centering
\begin{small}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        $i$ & Agent & Vertex & $t_i$ & $Q^{(i)}$ & $d(Q^{(i)} , Exit)$ & Cost \\
        \hline
        1 & $S_1$ & $V_4$ & 0 & $V_8$ & $\sqrt{2-2\cos\left(\tfrac{8\pi}{9}\right)}$ & \\
        \hline
        2 & $S_2$ & $V_5$ & 0 & $V_8$ & $\sqrt{3}$ &  \\
        \hline
        3 & $Q$ & $V_8$ & 0 & $V_8$ & 0 & \\
        \hline
        4 & $S_1$ & $V_3$ & $e_9$ & $(x_{2,9},0)$ & $\sqrt{x_{2,9}^2+x_{2,9}+1}$ & $^*$\\
        \hline
        5 & $S_2$ & $V_6$ & $e_9$ & $(x_{2,9},0)$ & $\sqrt{x_{2,9}^2+x_{2,9}+1}$ &  $^*$\\
        \hline
        6 & $Q$ & $V_9$ & $e_9+1-x_{2,9}$ & $V_9$ & 0 & \\
        \hline
        7 & $S_1$ & $V_2$ & $2e_9$ & $(y_{2,9},0)$ & $\sqrt{y_{2,9}^2-2y_{2,9}\cos\left(\tfrac{4\pi}{9}\right)+1}$ & $^*$ \\
        \hline
        8 & $S_2$ & $V_7$ & $2e_9$ & $(y_{2,9},0)$ & $\sqrt{y_{2,9}^2-2y_{2,9}\cos\left(\tfrac{4\pi}{9}\right)+1}$ & $^*$\\
        \hline
        9 & $Q$ & $V_1$ & $2e_9+\sqrt{y_{2,9}^2-2y_{2,9}\cos\left(\tfrac{2\pi}{9}\right)+1}$ & $V_1$ & 0 & \\
        \hline 
    \end{tabular}
\end{small}
\caption{Trajectories' details for the upper bound of \pe{9}{2}; 
see Figure~\ref{9gonk2fig}.}
\label{9gonk2tab}
\end{table}


==> UpperBoundsTabs/k3servants/3gonk3tab.tex <==
\begin{table}[h!]
\centering
\caption{Trajectories' details for the upper bound of \pe{3}{3}; 
see Figure~\ref{3gonk3fig}.}
\label{3gonk3tab}
\end{table}


==> UpperBoundsTabs/k4servants/10gonk4tab-old.tex <==
\begin{table}[h!]
\centering
\begin{small}
\begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        $i$ & Agent & Vertex & $t_i$ & $Q^{(i)}$ & $d(Q^{(i)} , Exit)$ & Cost \\
        \hline
        1 & $S_1$ & $V_1$ & 0 & $\cal{O}$ & 1 & 1 \\
        \hline
        2 & $S_2$ & $V_3$ & 0 & $\cal{O}$ & 1 & 1 \\
        \hline
        3 & $S_3$ & $V_5$ & 0 & $\cal{O}$ & 1 & 1 \\
        \hline
        4 & $S_4$ & $V_9$ & 0 & $\cal{O}$ & 1 & 1 \\
        \hline
        5 & $S_1$ & $V_2$ & $e_{10}$ & $\cal{O}$ & 1 & $1+e_{10}$  \\
        \hline
        6 & $S_2$ & $V_4$ & $e_{10}$ & $\cal{O}$ & 1 & $1+e_{10}$  \\
        \hline
        7 & $S_3$ & $V_6$ & $e_{10}$ & $\cal{O}$ & 1 & $1+e_{10}$  \\
        \hline
        8 & $S_4$ & $V_{10}$ & $e_{10}$ & $\cal{O}$ & 1 & $1+e_{10}$  \\
        \hline
        9 & $S_3$ & $V_7$ & $2e_{10}$ & $(0,-e_{10})$ & $x_{4,10}$ & $2e_{10}+x_{4,10}$ $^*$ \\
        \hline 
        10 & $Q$ & $V_8$ & $2e_{10}+x_{4,10}$ & $V_8$ & 0 & $2e_{10}+x_{4,10}$ $^*$ \\
        \hline 
    \end{tabular}
\end{small}
\caption{Trajectories' details for the upper bound of \pe{10}{4}; 
see Figure~\ref{10gonk4fig}.}
\label{10gonk4tab}
\end{table}

==> UpperBoundsTabs/k4servants/3gonk4tab.tex <==
\begin{table}[h!]
\centering
\caption{Trajectories' details for the upper bound of \pe{3}{4}; 
see Figure~\ref{3gonk4fig}.}
\label{3gonk4tab}
\end{table}


==> UpperBoundsTabs/k4servants/4gonk4tab.tex <==
\begin{table}[h!]
\centering
\caption{Trajectories' details for the upper bound of \pe{4}{4}; 
see Figure~\ref{4gonk4fig}.}
\label{4gonk4tab}
\end{table}

